Heisenberg-Langevin Formalism For Open Circuit-QED Systems

We present a Heisenberg-Langevin formalism to study the effective dynamics of a superconducting qubit coupled to an open multimode resonator, without resorting to the rotating wave, two level, Born or Markov approximations. Our effective equations are derived by eliminating resonator degrees of freedom while encoding their effect in the Green's function of the electromagnetic background. We account for the openness of the resonator exactly by employing a spectral representation for the Green's function in terms of a set of non-Hermitian modes. A well-behaved time domain perturbation theory is derived to systematically account for the nonlinearity of weakly nonlinear qubits like transmon. We apply this method to the problem of spontaneous emission, capturing accurately the non-Markovian features of the qubit dynamics, valid for any qubit-resonator coupling strength. Any discrete-level quantum system coupled to the electromagnetic continuum is subject to radiative decay and renormalization of its energy levels. When inside a cavity, these quantities can be strongly modified with respect to vacuum. Generally, this modification can be captured by including only the closest resonant cavity mode. In circuit-QED architecture, with substantial coupling strengths, it is however found that such rates are strongly influenced by far off-resonant modes. A multimode calculation over the infinite set of cavity modes leads to divergences unless an artificial cutoff is imposed. Previous studies have not pointed out what the source of this divergence is. We show that unless the effect of $A^2$ is accounted for up to all orders exactly, any multimode calculations of circuit-QED quantities is bound to diverge. Subsequently, we present the calculation of finite radiative corrections to qubit properties that is free of an artificially introduced high frequency cut-off.

==> Ch-Appendices/MultimodeJC.tex <==
\chapter{Multimode Jaynes-Cummings Hamiltonian}
The classical Hamiltonian for the cQED system can be found from the circuit Lagrangian~(\ref{Eq:Full Lagrangian}) \cite{Malekakhlagh_Origin_2016}
\begin{align}
\begin{split}
\mathcal{H}_{sys}&=4\mathcal{E}_c n_j^2(t)-\mathcal{E}_j\cos{[\varphi_j(t)]}\\
&+\int_{0}^{1}dx \left\{\frac{n^2(x,t)}{2\chi(x,x_0)}+\frac{1}{2}\left[\partial_x \varphi(x,t)\right]^2\right\}\\
&+2\pi\gamma z n_j(t)\int_{0}^{1}dx\frac{n(x,t)}{\chi(x,x_0)}\delta(x-x_0),
\end{split}
\label{eqn:model-closed cQED H}
\end{align}
where $z\equiv Z/R_Q$ where $Z\equiv\sqrt{l/c}$ is the characteristic impedance of the resonator and $R_Q\equiv h/(2e)^2$ is the superconducting resistance quantum. The modification in capacitance per length originates from the system Lagrangian that contains the gauge-invariant qubit-resonator coupling $\chi_g[\dot{\varphi}_j(t)-\dot{\varphi}(x_0,t)]^2/2$. In contrast, a phenomenological product coupling $\chi_g\dot{\varphi}_j(t)\dot{\varphi}(x_0,t)$ would yield a $\mathcal{H}_{sys}$ with $\chi_s=0$ which results in bare resonator modes.

For the purpose of quantizing $\mathcal{H}_{sys}$, we find the spectrum of the resonator by solving the corresponding Helmholtz eigenvalue problem that has been discussed in Sec.~(\ref{SubApp:Spec Rep of G-closed}). We find

\begin{align}
\hat{\mathcal{H}}_{\text{sys}} \equiv \frac{\omega_j}{4}\left\{\hat{\mathcal{Y}}_j^2-\frac{\sqrt{2}}{\epsilon}\cos\left[(2\epsilon^2)^{1/4}\hat{\mathcal{X}}_j\right]\right\}+\sum\limits_{n}\left\{\frac{\omega_n}{4}\left[\hat{\mathcal{X}}_n^2+\hat{\mathcal{Y}}_n^2\right]+g_n\hat{\mathcal{Y}}_j\hat{\mathcal{Y}}_n\right\},
\label{Eq:2nd quantized closed H}
\end{align}
where have defined the canonically conjugate variables $\hat{\mathcal{X}}_l\equiv(\hat{a}_l+\hat{a}_l^{\dag})$ and $\hat{\mathcal{Y}}_l\equiv -i(\hat{a}_l-\hat{a}_l^{\dag})$, where $\hat{a}_{l}$ represent the boson annihilation operator of sector $l\equiv j,c$. Moreover, $\omega_j\equiv \sqrt{8\mathcal{E}_j\mathcal{E}_c}$ and $\epsilon\equiv\sqrt{\mathcal{E}_c/\mathcal{E}_j}$ is a measure for the strength of transmon nonlinearity. For $\epsilon=0$, we recover $\omega_j(\hat{\mathcal{X}}_j^2+\hat{\mathcal{Y}}_j^2)/4$, the Hamiltonian of a simple harmonic oscillator. In the transmon regime where $\epsilon\ll 1$, the leading contribution is $-\sqrt{2}\epsilon\omega_j\hat{\mathcal{X}}_j^4/48$. The coupling between qubit and the $n$th CC mode of the resonator is
\begin{align} 
g_n=\frac{1}{2}\gamma\sqrt{\chi_j}\sqrt{\omega_j\omega_n}\tilde{\varphi}_n(x_0).
\label{eqn:Light-Matter g_n} 
\end{align}

There are typically two approaches to diagonalize Eq.~(\ref{Eq:2nd quantized closed H}). In the first approach, assuming that the qubit nonlinearity is strong, one performs a two level reduction. Then, the multimode Rabi Hamiltonian can be derived from Eq.~(\ref{Eq:2nd quantized closed H}) by projecting the quadratures to Pauli sigma matrices, $\hat{\mathcal{X}}_j\rightarrow\hat{\sigma}^x$ and $\hat{\mathcal{Y}}_j\rightarrow\hat{\sigma}^y$, which yields
\begin{align}
\hat{\mathcal{H}}_{\text{Rabi}}=\frac{\omega_j}{2}\hat{\sigma}^z+\sum\limits_{n}\omega_n\hat{a}_n^{\dag}\hat{a}_n-\sum\limits_ng_n(\hat{a}_n-\hat{a}_n^{\dag})(\hat{\sigma}^--\hat{\sigma}^+).
\label{Eq:Rabi H}
\end{align}
In the rotating wave approximation, Eq.~(\ref{Eq:Rabi H}) transforms into the multimode Jaynes-Cummings Hamiltonian
\begin{align}
\hat{\mathcal{H}}_{\text{JC}}=\frac{\omega_j}{2}\hat{\sigma}^z+\sum\limits_{n}\omega_n\hat{a}_n^{\dag}\hat{a}_n+\sum\limits_ng_n(\hat{\sigma}^+\hat{a}_n+\hat{\sigma}^-\hat{a}_n^{\dag})
\label{Eq:JC H}
\end{align}
used in the main text. Analytic results can be found for the Purcell decay rate and the Lamb shift in the dispersive limit where $g_n\ll|\omega_j-\omega_n|$ \cite{Boissonneault_Dispersive_2009}. In a Lindblad calculation, resonator losses are included by a Bloch-Redfield approach through the Master equation for the reduced density matrix of the resonator and qubit degrees of freedom $\hat{\dot{\rho}} = -i [ \hat{\mathcal{H}}_\text{JC}, \hat{\rho} ] + \frac{\kappa_n}{2} \left( 2 \hat{a}_n \hat{\rho} \hat{a}_n^\dagger - \{ \hat{\rho}, \hat{a}_n^\dagger \hat{a}_n \} \right)$, where $\kappa_n$ can be replaced from the solutions to Eq.~(\ref{Eq:Generic NHEigfreq}). The second approach treats the nonlinearity as a weak perturbation and is explained in the next section.

==> Ch-Appendices/cQEDNotation.tex <==
\chapter{cQED Notation}
\label{App:cQEDNotation}

In order to describe the dynamics of any cQED system we follow a common quantization procedure \cite{Bishop_Circuit_2010, Devoret_Quantum_2014}. The first step is to write the Lagrangian in terms of a generalized coordinate $\mathcal{L}[q_n]$. Then, a Legendre transformation to find the Hamiltonian in terms of the coordinate and its conjugate momentum $p_n\equiv \frac{\partial \mathcal{L}}{\partial \dot{q}_n}$ as $\mathcal{H}[q_n,p_n]=\sum\limits_n \dot{q}_n p_n -\mathcal{L}$ . Finally, we need to apply the canonical quantization by imposing a nonzero commutation relation between the conjugate pairs as  $[q_n,p_n]=i\hbar $. Here we go after the convention used in cQED by choosing the generalized coordinate as $\Phi_n(t)=\int_0^t V_n(t')\,dt'\ $ in which $V_n(t)$ is the voltage at node $n$ and is measured with respect to a ground node. This quantity has the units of magnetic flux and it can be shown that its conjugate variable has the units of charge and we denote it by $Q_n(t)$. 
There is an additional rule one has to keep in mind. In the case of external magnetic flux applied on a certain loop, the algebraic sum of flux variables over that loop should be equal to the external flux. Taking into account all these considerations, the Lagrangian for any cQED system is found as
\begin{align}
\mathcal{L}[\Phi_n ,\dot{\Phi}_n]=\mathcal{T}[\dot{\Phi}_n ]-\mathcal{U}[\Phi_n]
\end{align}
where $\mathcal{T}$ represents the kinetic energy corresponding to capacitors as $ \mathcal{T}_C[\dot{\Phi}]=\frac{1}{2}C\dot{\Phi}_C^2 $ and $\mathcal{U}$ stands for the potential energy corresponding to inductors as $ \mathcal{U}_L\{\Phi\}=\frac{1}{2L}\Phi_L^2 $ or any other nonlinear magnetic device such as Josephson junction $ \mathcal{U}_{J}[\Phi_J]=-E_J\cos\left(2\pi\frac{\Phi_J}{\phi_0}\right)$ where $\phi_0=\frac{h}{2e}$ is the flux quantum.

==> Ch-Publications/ConferencePresentations.tex <==
\chapter*{Conference Presentations}
\label{App:ConfPres}
\begin{enumerate}

\item Moein Malekakhlagh, Alexandru Petrescu and Hakan E. T\"ureci, "Non-Markovian dynamics of superconducting qubit in open multimode resonator", APS March Meeting, 2017

\item Moein Malekakhlagh, Alexandru Petrescu and Hakan E. T\"ureci, "Convergent expressions for Purcell rate and Lamb shift of superconducting qubit in an open multimode resonator", APS March Meeting, 2017

\item Moein Malekakhlagh, Hakan E. T\"ureci, "Origin and Implications of $A^2$-Contribution in the Quantization of Circuit-Qed Systems", APS March Meeting, 2016

\item Neereja Sundaresan, Yanbing Liu, Darius Sadri, Laszlo Szocs, Devin Underwood, Moein Malekakhlagh, Hakan E. T\"ureci, Andrew Houck, "Multimode Strong Coupling in Circuit QED", APS March Meeting, 2016

\item Moein Malekakhlagh, Neereja Sundaresan, Yanbing Liu, Darius Sadri, Andrew Houck, Hakan E. T\"ureci, "Amplitude Bistability in the Multimode Regime of Circuit-QED", APS March Meeting, 2015

\item Moein Malekakhlagh, Hakan E. T\"ureci, Dmitry Krimer, Matthias Liertzer, Stefan Rotter, "Non-Markovian Qubit Dynamics in Multimode Superconducting circuit cavities", APS March Meeting, 2014
\end{enumerate}
